Constructing Mutually Unbiased Bases from Quantum Latin Squares

We introduce orthogonal quantum Latin squares, which restrict to traditional orthogonal Latin squares, and investigate their application in quantum information science. We use quantum Latin squares to build maximally entangled bases, and show how a pair of mutually unbiased maximally entangled bases can be constructed in square dimension from orthogonal quantum Latin squares. We also compare our construction to an existing construction due to Beth and Wocjan and show that ours is strictly more general.

==> eptcsdata.tex <==
\providecommand{\firstpage}{108}
\providecommand{\publicationstatus}{R. Duncan and C. Heunen (Eds.): Quantum Physics and Logic (QPL) 2016\\
EPTCS 236, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.236.8}{10.4204/EPTCS.236.8}}

